Positive Definite Kernels and Random Sequences Connected to Polynomial Hypergroups

This work explores new classes of nonstationary stochastic sequences associated with polynomial hypergroups. Their covariance structures are analyzed through positive definite kernels and corresponding Hilbert spaces. Novel consistent estimators are introduced for deriving covariance structures from sequence realizations. A comprehensive prediction theory is developed, including a fast Levinson-type algorithm for efficiently calculating best linear predictors. Wiener-type theorems are established, enabling the detection of spectral measure atoms via generalized periodograms. Additional advancements, such as prediction with supplementary information, further enhance the scope of this study.

==> HyperProcess.tex <==

\begin{definition}
A sequence $(X_n)_{\nin_0}$ of square integrable (complex-valued)
random variables on a probability space $(\Omega,P)$ is called
{\bf weakly stationary on the \mbox{ polynomial} hypergroup
$\mathbf{{\Bbb N}_0}$ induced by $\mathbf{(R_n)_{\nin_0}}$}
provided the function $\;{d(m,n):= E(X_m \overline{X_n})\;}$ is
bounded and fulfils
\begin{equation}
d(m,n) \; = \; \sum_{k=|m-n|}^{m+n} g(m,n;k)\; d(k,0).
\end{equation}
\end{definition}
We will write $d(m)$ instead of $d(m,0).\;$ Notice that we do not
make any assumptions on the mean values $E(X_n).\;$ Obviously
$d(m,n)$ is the usual covariance only if $E(X_n) =0$ for all
$\nin_0.\;$ Now it is easily shown that $(d(n))_{\nin_0}$ is a
bounded positive definite sequence in the sense of (7). Hence
there exists a unique bounded positive Borel measure $\mu$ on
$D_s$ such that for all $\nin_0$
\begin{equation}
E(X_k \overline{X_0}) \; = \; d(k) \; = \; \int_{D_s} R_k(x) \;
d\mu (x), \qquad k \in {\Bbb N}_0.
\end{equation}
We call $\mu$ the spectral measure of $(X_n)_{\nin_0}.\;$
Combining (1) and (8) we get from (9) for all $n,m \in {\Bbb N}_0$
\begin{equation}
E(X_m \overline{X_n}) \; = \; d(m,n) \; = \; \int_{D_s} R_m(x) \;
R_n (x) \; d\mu (x),
\end{equation}
showing that $(X_n)_{\nin_0}$ belongs to the Karhunen class.
Moreover a Cramer representation theorem is valid. A
straightforward modification of known arguments yields an
orthogonal stochastic measure $ Z : {\cal B} \rightarrow
L^2(P),\;\; {\cal B}$ being the Borel $\sigma$-algebra on $D_s$
such that
\begin{equation}
X_k \; = \; \int_{D_s} R_k(x) \; dZ(x),
\end{equation}
where $\parallel Z(A)\parallel_2^2 \; = \mu (A) \;$ for all $A \in
{\cal B}.$

In fact the following characterizations of weak stationarity hold.

\begin{theorem}
For $(X_n)_{\nin_0} \subset L^2(\Omega,P)$ the following
statements are equivalent:
\begin{enumerate}
\item[(i)] $(X_n)_{\nin_0}$ is weakly stationary on the polynomial
hypergroup ${\Bbb N}_0$ induced by $(R_n)_{\nin_0}.$ \item[(ii)]
$E(X_m \overline{X_n})\;=\;\displaystyle\int_{D_s}
R_m(x)\;R_n(x)\;d\mu (x) \quad$ for every $n,m \in {\Bbb N}_0,\;$
where $\mu$ is a bounded positive Borel measure on $D_s.$
\item[(iii)] $X_k=\displaystyle\int_{D_s} R_k(x) \; dZ(x) \quad$
for every $k \in {\Bbb N}_0,\;$ where $Z$ is an orthogonal
stochastic measure on $D_s$.
\end{enumerate}
\end{theorem}

\begin{proof}
$(i) \Rightarrow (ii)\;$ is already shown. $(ii) \Rightarrow (iii)
\;$ is based on the isometric isomorphism $\Phi$ between
$L^2(D_s,\mu)$ and $H = $ span $ \{ X_n: \nin_0 \}^- \subseteq
L^2(\Omega,P) \;$ determined by $\; \Phi (R_n) = X_n.\;$ The
stochastic measure is defined by $Z(A)=\Phi(\chi_A),\;\;A $ being
a Borel subset of $D_s.\;$ The construction parallels the
classical case (see Shiryayev (1984, 395-403)).

Finally, assuming $(iii)$ we get for every $m,n \in {\Bbb N}_0$
$$ E(X_m \overline{X_n}) \;=\; \int_{D_s} R_m(x) \;R_n(x) \; d\mu(x),$$
where $\mu$ is defined by $\mu(A) \;= \parallel
Z(A)\parallel_2^2,\;\; A \in {\cal B}.\;$ The linearization of
$R_m(x)R_n(x)\;$ gives
$$ E(X_m \overline{X_n}) \;=\; \sum_{k=|n-m|}^{m+n} g(m,n;k)\; E(X_k\overline{X_0}).$$
\end{proof}


==> HyperSequence.tex <==
\begin{equation}
E(X_k \overline{X_0}) \; = \; d(k) \; = \; \int_{D_s} R_k(x) \;
d\mu (x), \qquad k \in {\Bbb N}_0.
\end{equation}
We call $\mu$ the spectral measure of $(X_n)_{\nin_0}.\;$
Combining (1) and (8) we get from (9) for all $n,m \in {\Bbb N}_0$
\begin{equation}
E(X_m \overline{X_n}) \; = \; d(m,n) \; = \; \int_{D_s} R_m(x) \;
R_n (x) \; d\mu (x),
\end{equation}
showing that $(X_n)_{\nin_0}$ belongs to the Karhunen class.
Moreover a Cramer representation theorem is valid. A
straightforward modification of known arguments yields an
orthogonal stochastic measure $ Z : {\cal B} \rightarrow
L^2(P),\;\; {\cal B}$ being the Borel $\sigma$-algebra on $D_s$
such that
\begin{equation}
X_k \; = \; \int_{D_s} R_k(x) \; dZ(x),
\end{equation}
where $\parallel Z(A)\parallel_2^2 \; = \mu (A) \;$ for all $A \in
{\cal B}.$

In fact the following characterizations of weak stationarity hold.

\begin{theorem}
For $(X_n)_{\nin_0} \subset L^2(\Omega,P)$ the following
statements are equivalent:
\begin{enumerate}
\item[(i)] $(X_n)_{\nin_0}$ is weakly stationary on the polynomial
hypergroup ${\Bbb N}_0$ induced by $(R_n)_{\nin_0}.$ \item[(ii)]
$E(X_m \overline{X_n})\;=\;\displaystyle\int_{D_s}
R_m(x)\;R_n(x)\;d\mu (x) \quad$ for every $n,m \in {\Bbb N}_0,\;$
where $\mu$ is a bounded positive Borel measure on $D_s.$
\item[(iii)] $X_k=\displaystyle\int_{D_s} R_k(x) \; dZ(x) \quad$
for every $k \in {\Bbb N}_0,\;$ where $Z$ is an orthogonal
stochastic measure on $D_s$.
\end{enumerate}
\end{theorem}

\begin{proof}
$(i) \Rightarrow (ii)\;$ is already shown. $(ii) \Rightarrow (iii)
\;$ is based on the isometric isomorphism $\Phi$ between
$L^2(D_s,\mu)$ and $H = $ span $ \{ X_n: \nin_0 \}^- \subseteq
L^2(\Omega,P) \;$ determined by $\; \Phi (R_n) = X_n.\;$ The
stochastic measure is defined by $Z(A)=\Phi(\chi_A),\;\;A $ being
a Borel subset of $D_s.\;$ The construction parallels the
classical case (see Shiryayev (\cite{Shir} 395-403)).

Finally, assuming $(iii)$ we get for every $m,n \in {\Bbb N}_0$
$$ E(X_m \overline{X_n}) \;=\; \int_{D_s} R_m(x) \;R_n(x) \; d\mu(x),$$
where $\mu$ is defined by $\mu(A) \;= \parallel
Z(A)\parallel_2^2,\;\; A \in {\cal B}.\;$ The linearization of
$R_m(x)R_n(x)\;$ gives
$$ E(X_m \overline{X_n}) \;=\; \sum_{k=|n-m|}^{m+n} g(m,n;k)\; E(X_k\overline{X_0}).$$
\end{proof}


==> PProcess.tex <==
Now, we come to the best investigated class, connected to
polynomial hypergroups: $P_n$-weakly stationary sequences. To get
consistency with the existing literature,  we use here the
notations $d(n,m)=K(n,m)$ and $d(n)=K(n,0)$.
\begin{Definition}
A sequence $(X_n)_{\nin}$ of square integrable (complex-valued)
random variables on a probability space $(\Omega,P)$ is called
weakly stationary on the polynomial hypergroup ${\Bbb N}_0$
induced by $(P_n)_{\nin}$ provided the function $\;{d(m,n):= E(X_m
\overline{X_n})\;}$ is bounded and fulfils
\begin{equation}
d(m,n) \; = \; \sum_{k=|m-n|}^{m+n} g(m,n,k)\; d(k,0).
\end{equation}
\end{Definition}
Since we use centered processes, we impose no assumptions on the
mean values $E(X_n)$. In general, one requires constant means.
Obviously, $d(m,n)$ is the usual covariance only if $E(X_n) =0$
for all $\nin.\;$ Now it is easily shown that $(d(n))_{\nin}$ is a
bounded positive definite sequence in the sense of
(\ref{Hyperposdef}). Hence there exists a unique bounded positive
Borel measure $\mu$ on $D_s$ such that for all $\nin$
\begin{equation}
E(X_k \overline{X_0}) \; = \; d(k) \; = \; \int_{D_s} P_k(x) \;
d\mu (x), \qquad k \in {\Bbb N}_0.
\end{equation}
We call $\mu$ the spectral measure of $(X_n)_{\nin}.\;$ According
to (\ref{SpecK}) we get for all $n,m \in {\Bbb N}_0$
\begin{equation}
E(X_m \overline{X_n}) \; = \; d(m,n) \; = \; \int_{D_s} P_m(x) \;
P_n (x) \; d\mu (x),
\end{equation}
showing that $(X_n)_{\nin}$ belongs to the Karhunen class
((\cite{ChaRao}, p.59). Moreover a Cramer representation theorem
(see \cite{CraHilb}) is valid. A straightforward modification of
known arguments yields an orthogonal stochastic measure $ Z :
{\cal B} \rightarrow L^2(P),\;\; {\cal B}$ being the Borel
$\sigma$-algebra on $D_s$ such that
\begin{equation}
X_k \; = \; \int_{D_s} P_k(x) \; dZ(x),
\end{equation}
where $\parallel Z(A)\parallel_2^2 \; = \mu (A) \;$ for all $A \in
{\cal B}.$

In fact the following characterizations of weak stationarity hold.

\begin{Theorem}\label{charHypostation}
For $(X_n)_{\nin} \subset L^2(\Omega,P)$ the following statements
are equivalent:
\begin{enumerate}
\item[(i)] $(X_n)_{\nin}$ is weakly stationary on the polynomial
hypergroup ${\Bbb N}_0$ induced by $(P_n)_{\nin}.$ \item[(ii)]
$E(X_m \overline{X_n})\;=\;\displaystyle\int_{D_s}
P_m(x)\;P_n(x)\;d\mu (x) \quad$ for every $n,m \in {\Bbb N}_0,\;$
where $\mu$ is a bounded positive Borel measure on $D_s.$
\item[(iii)] $X_k=\displaystyle\int_{D_s} P_k(x) \; dZ(x) \quad$
for every $k \in {\Bbb N}_0,\;$ where $Z$ is an orthogonal
stochastic measure on $D_s$.
\end{enumerate}
\end{Theorem}

\begin{proof}
$(i) \Rightarrow (ii)\;$ is already shown. $(ii) \Rightarrow (iii)
\;$ is based on the isometric isomorphism $\Phi$ between
$L^2(D_s,\mu)$ and $H = \overline {span \{ X_n: \nin \}} \subseteq
L^2(\Omega,P) \;$ determined by $\; \Phi (P_n) = X_n.\;$ The
stochastic measure is defined by $Z(A)=\Phi(\chi_A),\;\;A $ being
a Borel subset of $D_s.\;$ The construction parallels the
classical case (see Shiryayev (\cite{Shir}, 395-403)).

Finally, assuming $(iii)$ we get for every $m,n \in {\Bbb N}_0$
$$ E(X_m \overline{X_n}) \;=\; \int_{D_s} P_m(x) \;P_n(x) \; d\mu(x),$$
where $\mu$ is defined by $\mu(A) \;= \parallel
Z(A)\parallel_2^2,\;\; A \in {\cal B}.\;$ The linearization of
$P_m(x)P_n(x)\;$ gives
$$ E(X_m \overline{X_n}) \;=\; \sum_{k=|n-m|}^{m+n} g(m,n,k)\; E(X_k\overline{X_0}).$$
\end{proof}

Consider now on the Hilbert space $H$ the linear operators
$$\displaystyle T_n(X_m) := \sum_{s=|m-n|}^{n+m} g(n,m,s) X_s$$.
Linear continuation of $T_n$ in $H$ yields shift operators which
are normal, are all commutating and satisfy \cite{lalest}
\begin{equation}\label{shifts}
    T_n \cdot T_m = \sum_{s=|n-m|}^{n+m} g(n,m,s) T_s.
\end{equation}


==> cyclo.tex <==
An important generalization of weakly stationary processes are
periodically correlated (cyclostationary) processes and almost
periodically correlated processes. The definitions were introduced
by Gladyshev \cite{Glad}

